Community Empowerment through Location-Based AR: The Th\'amien Ohlone AR Tour

Community empowerment is the process of enabling communities to increase control over their narratives, resources, and futures. In HCI and design, this social challenge centers on helping marginalized groups gain agency through technology and design interventions. For Indigenous communities in particular, empowerment means not only representation but sovereignty in how their stories are told and by whom. Location-based augmented reality (AR) offers a novel opportunity to address this challenge. By overlaying digital content onto physical places, AR can spatially anchor community narratives in the real world, allowing communities to re-tell the story of a place on their own terms. Such site-specific AR experiences have already been used to reveal hidden histories, re-imagine colonial monuments, and celebrate minority cultures. The affordances of XR - particularly AR\'s spatial interaction and immersive storytelling - make it a promising tool for cultural continuity and community activism. In this position paper, we focus on how these XR affordances can empower communities, using the Th\'amien Ohlone AR Tour as a case study. We outline why traditional digital interventions fall short of true empowerment, how AR's immersive qualities uniquely support Indigenous self-determination, insights from co-designing the Ohlone AR Tour, and future directions to scale such efforts responsibly.

==> trash.tex <==

Others explore switching the interface to achieve the goals. Depending on how adaptation responsibility is allocated, there are three key types of adaptation: Adaptive user interfaces (Adaptive UI) automatically adjust the user interface in response to contextual changes~\cite{Harman2014, Oreizy1999}. Adaptable user interfaces (Adaptable UI) allow users to tailor the UI components to their needs~\cite{Zhang2019, Perez2018}. 
add semi-adptive here

 \citet{Romero2020} focused on the long-term use of Adaptable UI in mobile transit information to examine the impact of adaptation. Their findings provide evidence that a well-performing Adaptable UI leads to reduced interaction effort, while poor performance may lead to more interaction effort than no adaptation.

Therefore, we propose an adaptable approach that provides parents and teens with flexibility based on the parents’ advising style, as well as their agreements and communication. 

Other research was conducted by \citet{Sathya2024} have designed Attention Receipts — artifacts that materialize the time spent watching YouTube videos and found a positive correlation between the materiality of these receipts and participants' time spent consuming online media. 

Because of these existing gaps in research, it is important to find a way for parents and teens to collaborate on screen time management.
